Real-E: A Foundation Benchmark for Advancing Robust and Generalizable Electricity Forecasting

Energy forecasting is vital for grid reliability and operational efficiency. Although recent advances in time series forecasting have led to progress, existing benchmarks remain limited in spatial and temporal scope and lack multi-energy features. This raises concerns about their reliability and applicability in real-world deployment. To address this, we present the Real-E dataset, covering over 74 power stations across 30+ European countries over a 10-year span with rich metadata. Using Real- E, we conduct an extensive data analysis and benchmark over 20 baselines across various model types. We introduce a new metric to quantify shifts in correlation structures and show that existing methods struggle on our dataset, which exhibits more complex and non-stationary correlation dynamics. Our findings highlight key limitations of current methods and offer a strong empirical basis for building more robust forecasting models

==> tab1.tex <==
% \begin{table}[h]
% \centering
% \tiny
% \renewcommand{\arraystretch}{0.85}
% \caption{Comparing with existing datasets, \data offers longer duration (Dur.), finer resolution (Res.), longer sequences (Len.), more energy categories (EC) and broader country coverage (C).}
% \vspace{-2em}
% \label{tab:data-compare}
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{@{}c@{\hskip 4pt}l@{\hskip 4pt}c@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 3pt}c@{}}
% \toprule
% & \textbf{Name} & \textbf{Dur.} & \textbf{Res.} & \textbf{Len.} & \textbf{EC} & \textbf{C} \\
% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{0}{\parbox{1.5cm}{\centering\fontsize{6}{6}\selectfont\textcolor{gray}{\textbf{Existing\\Benchmark}}}}}
% %\midrule

% & \textcolor{gray}{Solar}       & \textcolor{gray}{1 y}    & \textcolor{gray}{10 min}  & \textcolor{gray}{52,560}  & \textcolor{gray}{1}  & \textcolor{gray}{1} \\
% & \textcolor{gray}{Electricity} & \textcolor{gray}{3 y}    & \textcolor{gray}{1 hour}  & \textcolor{gray}{26,304}  & \textcolor{gray}{1}  & \textcolor{gray}{1} \\

% & \textcolor{gray}{ETTh1/ETTh2}       & \textcolor{gray}{20 mon} & \textcolor{gray}{1 hour}  & \textcolor{gray}{14,400}  & \textcolor{gray}{1}  & \textcolor{gray}{1} \\
% & \textcolor{gray}{ETTm1/ETTm2}       & \textcolor{gray}{20 mon} & \textcolor{gray}{15 min}  & \textcolor{gray}{57,600}  & \textcolor{gray}{1}  & \textcolor{gray}{1} \\

% \midrule
% \multicolumn{7}{c}{\textbf{\data}} \\
% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{0}{Generation}} 
%   & \textcolor{teal}{Actual-ByType}      & \textcolor{teal}{9.5 y} & \textcolor{teal}{15 min}  & \textcolor{teal}{>330k}   & \textcolor{teal}{20} & \textcolor{teal}{39} \\
%   & Actual-ByUnit                        & 9.5 y & 1 hour  & ~8.7k   & 20 & 39 \\
%   & Renewables-Forecast                  & 9.5 y & 15 min  & >330k   & 3  & 39 \\
%   & Capacity-Annual                      & 9.5 y & 1 year  & ~10     & 20 & 39 \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{0}{Load}} 
%   & Actual                               & 9.5 y & 15 min  & >330k   & 20  & 39 \\
%   & Forecast-WeekAhead                   & 9.5 y & 1 day   & ~3.4k   & 20  & 39 \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{0}{Market}} 
%   & Price-QuarterHourly                  & 9.5 y & 15 min  & >330k   & 20 & 39 \\
%   & Price-Hourly                         & 9.5 y & 1 hour  & ~8.7k   & 20 & 39 \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{0}{Transmission}} 
%   & Capacity-Forecast                    & 9.5 y & 1 hour  & ~8.7k   & 20 & 39 \\
%   %& Flow-Scheduled                       & 9.5 y & 1 hour  & ~8.7k   & 20 & 39 \\
%   & Flow-Actual                          & 9.5 y & 1 hour  & ~8.7k   & 20 & 39 \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{0}{Balancing}} 
%   & Energy-Activated                     & 9.5 y & 15 min  & >330k   & 20 & 39 \\
%   & System-Imbalance                     & 9.5 y & 1 hour  & ~8.7k   & -- & 39 \\
% \bottomrule
% \end{tabular}%
% }
% \vspace{-4.0em}
% \end{table}



==> tab2_quantify.tex <==
\setlength{\abovecaptionskip}{0.2em}   % space above caption
\setlength{\belowcaptionskip}{-0.5em}  % space below caption

\begin{table}[!t]
\centering
\scriptsize
\caption{Average MAE and RMSE of 20 models on 4 datasets (forecasting horizon = 12).
\textbf{GR} (Gap Rank) is computed based on the performance gap between new and old datasets.} 
\label{tab:results_mae_rmse}
\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{1.7pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|cccccccc|>{\raggedleft\arraybackslash}p{0.18cm}}
\toprule
\textbf{Model} 
& \multicolumn{2}{c}{\textcolor{darkgray}{\textbf{Electricity}}} 
& \multicolumn{2}{c}{\textcolor{darkgray}{\textbf{Solar}}} 
& \multicolumn{2}{c}{\textbf{Germany}} 
& \multicolumn{2}{c}{\textbf{France}} 
& \multirow{2}{*}{\textcolor{teal}{\textbf{GR}}} \\
              & \textcolor{darkgray}{MAE} & \textcolor{darkgray}{RMSE} 
              & \textcolor{darkgray}{MAE} & \textcolor{darkgray}{RMSE} 
              & MAE & RMSE 
              & MAE & RMSE 
              &  \\
\midrule
\multicolumn{10}{l}{\textbf{Statistic Methods}} \\
S-ARIMA \cite{box2015time} & \textcolor{darkgray}{0.101} & \textcolor{darkgray}{0.163} & \textcolor{darkgray}{0.184} & \textcolor{darkgray}{0.234} & 0.268 & 0.379 & 0.158 & 0.273 & \textcolor{teal}{7} \\
ARIMA \cite{box2015time} & \textcolor{darkgray}{0.107} & \textcolor{darkgray}{0.169} & \textcolor{darkgray}{0.185} & \textcolor{darkgray}{0.244} & 0.275 & 0.319 & 0.164 & 0.281 & \textcolor{teal}{17} \\
VAR \cite{sims1980macroeconomics} & \textcolor{darkgray}{0.096} & \textcolor{darkgray}{0.155} & \textcolor{darkgray}{0.175} & \textcolor{darkgray}{0.222} & 0.243 & 0.381 & 0.177 & 0.260 & \textcolor{teal}{12} \\
\midrule
\multicolumn{10}{l}{\textbf{MLP-based}} \\
DLinear \cite{zeng2023dlinear} & \textcolor{darkgray}{0.058} & \textcolor{darkgray}{0.092} & \textcolor{darkgray}{0.257} & \textcolor{darkgray}{0.313} & 0.266 & 0.368 & 0.196 & 0.259 & \textcolor{teal}{19} \\
N-Beats \cite{oreshkin2020nbeats} & \textcolor{darkgray}{0.111} & \textcolor{darkgray}{0.179} & \textcolor{darkgray}{0.202} & \textcolor{darkgray}{0.257} & 0.189 & 0.325 & 0.174 & 0.300 & \textcolor{teal}{16} \\
TimeMixer \cite{wang2024timemixer} & \textcolor{darkgray}{0.091} & \textcolor{darkgray}{0.147} & \textcolor{darkgray}{0.166} & \textcolor{darkgray}{0.211} & 0.181 & 0.314 & 0.167 & 0.279 & \textcolor{teal}{15} \\
\midrule
\multicolumn{10}{l}{\textbf{RNN/CNN-based}} \\
DeepGLO \cite{sen2019think} & {0.090} & \textcolor{darkgray}{0.131} & \textcolor{darkgray}{0.178} & \textcolor{darkgray}{0.400} & 0.264 & 0.372 & 0.181 & 0.246 & \textcolor{teal}{8} \\
LSTNet \cite{lai2018modeling} & \textcolor{darkgray}{0.075} & \textcolor{darkgray}{0.138} & \textcolor{darkgray}{0.148} & \textcolor{darkgray}{0.200} & 0.193 & 0.346 & 0.177 & 0.263 & \textcolor{teal}{10} \\
TCN \cite{bai2018empirical} & \textcolor{darkgray}{0.057} & \textcolor{darkgray}{0.083} & \textcolor{darkgray}{0.176} & \textcolor{darkgray}{0.222} & 0.187 & 0.287 & 0.172 & 0.260 & \textcolor{teal}{11} \\
SFM \cite{zhang2017stock} & \textcolor{darkgray}{0.086} & \textcolor{darkgray}{0.129} & \textcolor{darkgray}{0.161} & \textcolor{darkgray}{0.283} & 0.184 & 0.245 & 0.156 & 0.238 & \textcolor{teal}{5} \\
\midrule
\multicolumn{10}{l}{\textbf{Transformer-based}} \\
Reformer \cite{kitaev2020reformer} & \textcolor{darkgray}{0.078} & \textcolor{darkgray}{0.129} & \textcolor{darkgray}{0.234} & \textcolor{darkgray}{0.292} & 0.297 & 0.361 & 0.141 & 0.233 & \textcolor{teal}{14} \\
Informer \cite{zhou2021informer} & \textcolor{darkgray}{0.070} & \textcolor{darkgray}{0.119} & \textcolor{darkgray}{0.151} & \textcolor{darkgray}{0.199} & 0.283 & 0.324 & 0.129 & 0.215 & \textcolor{teal}{18} \\ 
FEDformer \cite{zhou2022fedformer} & \cellcolor{gray!30}\textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.055}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.081}} & \textcolor{darkgray}{\cellcolor{gray!15}\textbf{0.139}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.182}} & 0.271 & 0.396 & 0.220 & 0.291 & \textcolor{teal}{20} \\
Autoformer \cite{wu2021autoformer} & \cellcolor{gray!10}\textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.056}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.083}} & \textcolor{darkgray}{0.150} & \textcolor{darkgray}{0.193} & 0.204 & 0.376 & 0.167 & 0.267 & \textcolor{teal}{13} \\  
% Patchtst \cite{nie2023time} & \cellcolor{gray!10}\textcolor{darkgray}{\cellcolor{gray!15}\textbf{0.058}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.094}} & \cellcolor{gray!15}{0.130} & \cellcolor{gray!15}{0.234} & \cellcolor{gray!15}\textbf{0.147} & \cellcolor{gray!15}\textbf{0.233} & \cellcolor{gray!15}\textbf{0.119} & 0.211 & \textcolor{teal}{5} \\  
\midrule
\multicolumn{10}{l}{\textbf{Spectral GNN}} \\
LSGCN \cite{huang2020lsgcn}  & \textcolor{darkgray}{0.097} & \textcolor{darkgray}{0.125} & \textcolor{darkgray}{0.174} &  0.262 & 0.134 & 0.209 & 0.093 & 0.172 & \textcolor{teal}{-} \\
StemGNN \cite{cao2020spectral}  & \textcolor{darkgray}{0.070} & \textcolor{darkgray}{0.101} & \textcolor{darkgray}{0.176} & \textcolor{darkgray}{0.222} & 0.179 & 0.285 & \cellcolor{gray!15}\textbf{0.148} & \cellcolor{gray!15}\textbf{0.206} & \textcolor{teal}{6} \\
FourierGNN \cite{yi2023fouriergnn}  & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.051}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.077}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.120}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.162}} & \cellcolor{gray!15}\textbf{0.110} & \cellcolor{gray!15}\textbf{0.186} & \cellcolor{gray!15}\textbf{0.096} & \cellcolor{gray!15}\textbf{0.164} & \textcolor{teal}{4} \\
\midrule
\multicolumn{10}{l}{\textbf{Spatial GNN}} \\
TPGNN \cite{wu2019graph} & \textcolor{darkgray}{0.055} & \textcolor{darkgray}{0.080} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.123}} & \textcolor{darkgray}{0.214} & \cellcolor{gray!15}{0.099} & \cellcolor{gray!15}{\textbf{0.173}} & \cellcolor{gray!15}{\textbf{0.089}} & \cellcolor{gray!15}{\textbf{0.158}} & \textcolor{teal}{3} \\
MTGNN \cite{wu2020connecting} & \textcolor{darkgray}{0.077} & \textcolor{darkgray}{0.113} & \textcolor{darkgray}{0.151} & \textcolor{darkgray}{0.207} & \cellcolor{gray!30}\textbf{0.016} & \cellcolor{gray!30}{\textbf{0.034}} & \cellcolor{gray!60}\textbf{0.012} & \cellcolor{gray!60}{\textbf{0.023}} & \textcolor{teal}{2} \\
GWaveNet \cite{liu2022tpg} & \textcolor{darkgray}{0.094} & \textcolor{darkgray}{0.140} & \textcolor{darkgray}{0.183} & \textcolor{darkgray}{0.238} & \cellcolor{gray!60}\textbf{0.013} & \cellcolor{gray!60}{\textbf{0.028}} & \cellcolor{gray!60}\textbf{0.012} & \cellcolor{gray!30}{\textbf{0.025}} & \textcolor{teal}{1} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> table_performance_backup.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Average MAE and RMSE of 20 models on 4 datasets (forecasting horizon = 12).
\textbf{GR} (Gap Rank) is computed based on the performance gap between new and old datasets.} 
\label{tab:results_mae_rmse}
\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{1.7pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|cccccccc|>{\raggedleft\arraybackslash}p{0.18cm}}
\toprule
\textbf{Model} 
& \multicolumn{2}{c}{\textcolor{darkgray}{\textbf{Electricity}}} 
& \multicolumn{2}{c}{\textcolor{darkgray}{\textbf{Solar}}} 
& \multicolumn{2}{c}{\textbf{Germany}} 
& \multicolumn{2}{c}{\textbf{France}} 
& \multirow{2}{*}{\textcolor{teal}{\textbf{GR}}} \\
              & \textcolor{darkgray}{MAE} & \textcolor{darkgray}{RMSE} 
              & \textcolor{darkgray}{MAE} & \textcolor{darkgray}{RMSE} 
              & MAE & RMSE 
              & MAE & RMSE 
              &  \\
\midrule
\multicolumn{10}{l}{\textbf{Statistic Methods}} \\
S-ARIMA \cite{box2015time} & \textcolor{darkgray}{0.101} & \textcolor{darkgray}{0.163} & \textcolor{darkgray}{0.184} & \textcolor{darkgray}{0.234} & 0.268 & 0.379 & 0.158 & 0.273 & \textcolor{teal}{7} \\
ARIMA \cite{box2015time} & \textcolor{darkgray}{0.107} & \textcolor{darkgray}{0.169} & \textcolor{darkgray}{0.185} & \textcolor{darkgray}{0.244} & 0.275 & 0.319 & 0.164 & 0.281 & \textcolor{teal}{17} \\
VAR \cite{sims1980macroeconomics} & \textcolor{darkgray}{0.096} & \textcolor{darkgray}{0.155} & \textcolor{darkgray}{0.175} & \textcolor{darkgray}{0.222} & 0.243 & 0.381 & 0.177 & 0.260 & \textcolor{teal}{12} \\
\midrule
\multicolumn{10}{l}{\textbf{MLP-based}} \\
DLinear \cite{zeng2023dlinear} & \textcolor{darkgray}{0.058} & \textcolor{darkgray}{0.092} & \textcolor{darkgray}{0.257} & \textcolor{darkgray}{0.313} & 0.266 & 0.368 & 0.196 & 0.259 & \textcolor{teal}{19} \\
N-Beats \cite{oreshkin2020nbeats} & \textcolor{darkgray}{0.111} & \textcolor{darkgray}{0.179} & \textcolor{darkgray}{0.202} & \textcolor{darkgray}{0.257} & 0.189 & 0.325 & 0.174 & 0.300 & \textcolor{teal}{16} \\
TimeMixer \cite{wang2024timemixer} & \textcolor{darkgray}{0.091} & \textcolor{darkgray}{0.147} & \textcolor{darkgray}{0.166} & \textcolor{darkgray}{0.211} & 0.181 & 0.314 & 0.167 & 0.279 & \textcolor{teal}{15} \\
\midrule
\multicolumn{10}{l}{\textbf{RNN/CNN-based}} \\
DeepGLO \cite{sen2019think} & {0.090} & \textcolor{darkgray}{0.131} & \textcolor{darkgray}{0.178} & \textcolor{darkgray}{0.400} & 0.264 & 0.372 & 0.181 & 0.246 & \textcolor{teal}{8} \\
LSTNet \cite{lai2018modeling} & \textcolor{darkgray}{0.075} & \textcolor{darkgray}{0.138} & \textcolor{darkgray}{0.148} & \textcolor{darkgray}{0.200} & 0.193 & 0.346 & 0.177 & 0.263 & \textcolor{teal}{10} \\
TCN \cite{bai2018empirical} & \textcolor{darkgray}{0.057} & \textcolor{darkgray}{0.083} & \textcolor{darkgray}{0.176} & \textcolor{darkgray}{0.222} & 0.187 & 0.287 & 0.172 & 0.260 & \textcolor{teal}{11} \\
SFM \cite{zhang2017stock} & \textcolor{darkgray}{0.086} & \textcolor{darkgray}{0.129} & \textcolor{darkgray}{0.161} & \textcolor{darkgray}{0.283} & 0.184 & 0.245 & 0.156 & 0.238 & \textcolor{teal}{5} \\
\midrule
\multicolumn{10}{l}{\textbf{Transformer-based}} \\
Reformer \cite{kitaev2020reformer} & \textcolor{darkgray}{0.078} & \textcolor{darkgray}{0.129} & \textcolor{darkgray}{0.234} & \textcolor{darkgray}{0.292} & 0.297 & 0.361 & 0.141 & 0.233 & \textcolor{teal}{14} \\
Informer \cite{zhou2021informer} & \textcolor{darkgray}{0.070} & \textcolor{darkgray}{0.119} & \textcolor{darkgray}{0.151} & \textcolor{darkgray}{0.199} & 0.283 & 0.324 & 0.129 & 0.215 & \textcolor{teal}{18} \\ 
FEDformer \cite{zhou2022fedformer} & \cellcolor{gray!30}\textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.055}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.081}} & \textcolor{darkgray}{\cellcolor{gray!15}\textbf{0.139}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.182}} & 0.271 & 0.396 & 0.220 & 0.291 & \textcolor{teal}{20} \\
Autoformer \cite{wu2021autoformer} & \cellcolor{gray!10}\textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.056}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.083}} & \textcolor{darkgray}{0.150} & \textcolor{darkgray}{0.193} & 0.204 & 0.376 & 0.167 & 0.267 & \textcolor{teal}{13} \\  
% Patchtst \cite{nie2023time} & \cellcolor{gray!10}\textcolor{darkgray}{\cellcolor{gray!15}\textbf{0.058}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.094}} & \cellcolor{gray!15}{0.130} & \cellcolor{gray!15}{0.234} & \cellcolor{gray!15}\textbf{0.147} & \cellcolor{gray!15}\textbf{0.233} & \cellcolor{gray!15}\textbf{0.119} & 0.211 & \textcolor{teal}{5} \\  
\midrule
\multicolumn{10}{l}{\textbf{Spectral GNN}} \\
LSGCN \cite{huang2020lsgcn}  & \textcolor{darkgray}{0.097} & \textcolor{darkgray}{0.125} & \textcolor{darkgray}{0.174} &  0.262 & 0.134 & 0.209 & 0.093 & 0.172 & \textcolor{teal}{-} \\
StemGNN \cite{cao2020spectral}  & \textcolor{darkgray}{0.070} & \textcolor{darkgray}{0.101} & \textcolor{darkgray}{0.176} & \textcolor{darkgray}{0.222} & 0.179 & 0.285 & \cellcolor{gray!15}\textbf{0.148} & \cellcolor{gray!15}\textbf{0.206} & \textcolor{teal}{6} \\
FourierGNN \cite{yi2023fouriergnn}  & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.051}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.077}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.120}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.162}} & \cellcolor{gray!15}\textbf{0.110} & \cellcolor{gray!15}\textbf{0.186} & \cellcolor{gray!15}\textbf{0.096} & \cellcolor{gray!15}\textbf{0.164} & \textcolor{teal}{4} \\
\midrule
\multicolumn{10}{l}{\textbf{Spatial GNN}} \\
TPGNN \cite{wu2019graph} & \textcolor{darkgray}{0.055} & \textcolor{darkgray}{0.080} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.123}} & \textcolor{darkgray}{0.214} & \cellcolor{gray!15}{0.099} & \cellcolor{gray!15}{\textbf{0.173}} & \cellcolor{gray!15}{\textbf{0.089}} & \cellcolor{gray!15}{\textbf{0.158}} & \textcolor{teal}{3} \\
MTGNN \cite{wu2020connecting} & \textcolor{darkgray}{0.077} & \textcolor{darkgray}{0.113} & \textcolor{darkgray}{0.151} & \textcolor{darkgray}{0.207} & \cellcolor{gray!30}\textbf{0.016} & \cellcolor{gray!30}{\textbf{0.034}} & \cellcolor{gray!60}\textbf{0.012} & \cellcolor{gray!60}{\textbf{0.023}} & \textcolor{teal}{2} \\
GWaveNet \cite{liu2022tpg} & \textcolor{darkgray}{0.094} & \textcolor{darkgray}{0.140} & \textcolor{darkgray}{0.183} & \textcolor{darkgray}{0.238} & \cellcolor{gray!60}\textbf{0.013} & \cellcolor{gray!60}{\textbf{0.028}} & \cellcolor{gray!60}\textbf{0.012} & \cellcolor{gray!30}{\textbf{0.025}} & \textcolor{teal}{1} \\
\bottomrule
\end{tabular}%
}
\vspace{-2.8em}
\end{table}



==> upt_tab.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Average MAE and RMSE of 20 models on 4 datasets (forecasting horizon = 12).}
\label{tab:results_mae_rmse}
\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{1.7pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|cccccccc}
\toprule
\textbf{Model} 
& \multicolumn{2}{c}{\textcolor{darkgray}{\textbf{Electricity}}} 
& \multicolumn{2}{c}{\textcolor{darkgray}{\textbf{Solar}}} 
& \multicolumn{2}{c}{\textbf{Germany}} 
& \multicolumn{2}{c}{\textbf{France}} \\
              & \textcolor{darkgray}{MAE} & \textcolor{darkgray}{RMSE} 
              & \textcolor{darkgray}{MAE} & \textcolor{darkgray}{RMSE} 
              & MAE & RMSE 
              & MAE & RMSE \\
\midrule
\multicolumn{9}{l}{\textbf{Statistic Methods}} \\
S-ARIMA \cite{box2015time} & \textcolor{darkgray}{0.101} & \textcolor{darkgray}{0.163} & \textcolor{darkgray}{0.184} & \textcolor{darkgray}{0.234} & 0.268 & 0.379 & 0.158 & 0.273 \\
ARIMA \cite{box2015time} & \textcolor{darkgray}{0.107} & \textcolor{darkgray}{0.169} & \textcolor{darkgray}{0.185} & \textcolor{darkgray}{0.244} & 0.275 & 0.319 & 0.164 & 0.281 \\
VAR \cite{sims1980macroeconomics} & \textcolor{darkgray}{0.096} & \textcolor{darkgray}{0.155} & \textcolor{darkgray}{0.175} & \textcolor{darkgray}{0.222} & 0.243 & 0.381 & 0.177 & 0.260 \\
\midrule
\multicolumn{9}{l}{\textbf{MLP-based}} \\
DLinear \cite{zeng2023dlinear} & \textcolor{darkgray}{0.058} & \textcolor{darkgray}{0.092} & \textcolor{darkgray}{0.257} & \textcolor{darkgray}{0.313} & 0.266 & 0.368 & 0.196 & 0.259 \\
N-Beats \cite{oreshkin2020nbeats} & \textcolor{darkgray}{0.111} & \textcolor{darkgray}{0.179} & \textcolor{darkgray}{0.202} & \textcolor{darkgray}{0.257} & 0.189 & 0.325 & 0.174 & 0.300 \\
TimeMixer \cite{wang2024timemixer} & \textcolor{darkgray}{0.091} & \textcolor{darkgray}{0.147} & \textcolor{darkgray}{0.166} & \textcolor{darkgray}{0.211} & 0.181 & 0.314 & 0.167 & 0.279 \\
\midrule
\multicolumn{9}{l}{\textbf{RNN/CNN-based}} \\
DeepGLO \cite{sen2019think} & {0.090} & \textcolor{darkgray}{0.131} & \textcolor{darkgray}{0.178} & \textcolor{darkgray}{0.400} & 0.264 & 0.372 & 0.181 & 0.246 \\
LSTNet \cite{lai2018modeling} & \textcolor{darkgray}{0.075} & \textcolor{darkgray}{0.138} & \textcolor{darkgray}{0.148} & \cellcolor{gray!15} \textcolor{darkgray}{\textbf{0.200}} & 0.193 & 0.346 & 0.177 & 0.263 \\
TCN \cite{bai2018empirical} & \textcolor{darkgray}{0.057} & \textcolor{darkgray}{0.083} & \textcolor{darkgray}{0.176} & \textcolor{darkgray}{0.222} & 0.187 & 0.287 & 0.172 & 0.260 \\
SFM \cite{zhang2017stock} & \textcolor{darkgray}{0.086} & \textcolor{darkgray}{0.129} & \textcolor{darkgray}{0.161} & \textcolor{darkgray}{0.283} & 0.184 & 0.245 & 0.156 & 0.238 \\
\midrule
\multicolumn{9}{l}{\textbf{Transformer-based}} \\
Reformer \cite{kitaev2020reformer} & \textcolor{darkgray}{0.078} & \textcolor{darkgray}{0.129} & \textcolor{darkgray}{0.234} & \textcolor{darkgray}{0.292} & 0.297 & 0.361 & 0.141 & 0.233 \\
Informer \cite{zhou2021informer} & \textcolor{darkgray}{0.070} & \textcolor{darkgray}{0.119} & \textcolor{darkgray}{0.151} & \textcolor{darkgray}{0.199} & 0.283 & 0.324 & 0.129 & 0.215 \\ 
FEDformer \cite{zhou2022fedformer} & \cellcolor{gray!30}\textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.055}} & \textcolor{darkgray}{\cellcolor{gray!15}\textbf{0.081}} & \textcolor{darkgray}{\cellcolor{gray!15}\textbf{0.139}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.182}} & 0.271 & 0.396 & 0.220 & 0.291 \\
Autoformer \cite{wu2021autoformer} & \cellcolor{gray!10}\textcolor{darkgray}{\cellcolor{gray!15}\textbf{0.056}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.083}} & \cellcolor{gray!15} \textcolor{darkgray}{\textbf{0.150}} & \cellcolor{gray!15} \textcolor{darkgray}{\textbf{0.193}} & 0.204 & 0.376 & 0.167 & 0.267 \\
\midrule
\multicolumn{9}{l}{\textbf{Spectral GNN}} \\
LSGCN \cite{huang2020lsgcn}  & \textcolor{darkgray}{0.097} & \textcolor{darkgray}{0.125} & \textcolor{darkgray}{0.174} &  0.262 & 0.134 & 0.209 & 0.093 & 0.172 \\
StemGNN \cite{cao2020spectral}  & \textcolor{darkgray}{0.070} & \textcolor{darkgray}{0.101} & \textcolor{darkgray}{0.176} & \textcolor{darkgray}{0.222} & 0.179 & 0.285 & \cellcolor{gray!15}\textbf{0.148} & 0.206 \\
FourierGNN \cite{yi2023fouriergnn}  & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.051}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.077}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.120}} & \cellcolor{gray!60}\textcolor{darkgray}{\textbf{0.162}} & \cellcolor{gray!15}\textbf{0.110} & \cellcolor{gray!15}\textbf{0.186} & \cellcolor{gray!15}\textbf{0.096} & \cellcolor{gray!15}\textbf{0.164} \\
\midrule
\multicolumn{9}{l}{\textbf{Spatial GNN}} \\
TPGNN \cite{wu2019graph} &  \cellcolor{gray!30}\textcolor{darkgray}{\textbf{0.055}} & \cellcolor{gray!30}\textcolor{darkgray}{\textbf{0.080}} & \textcolor{darkgray}{\cellcolor{gray!30}\textbf{0.123}} & \textcolor{darkgray}{0.214} & \cellcolor{gray!15}{\textbf{0.099}} & \cellcolor{gray!15}{\textbf{0.173}} & \cellcolor{gray!15}{\textbf{0.089}} & \cellcolor{gray!15}{\textbf{0.158}} \\
MTGNN \cite{wu2020connecting} & \textcolor{darkgray}{0.077} & \textcolor{darkgray}{0.113} & \textcolor{darkgray}{0.151} & \textcolor{darkgray}{0.207} & \cellcolor{gray!30}\textbf{0.016} & \cellcolor{gray!30}{\textbf{0.034}} & \cellcolor{gray!60}\textbf{0.012} & \cellcolor{gray!60}{\textbf{0.023}} \\
GWaveNet \cite{liu2022tpg} & \textcolor{darkgray}{0.094} & \textcolor{darkgray}{0.140} & \textcolor{darkgray}{0.183} & \textcolor{darkgray}{0.238} & \cellcolor{gray!60}\textbf{0.013} & \cellcolor{gray!60}{\textbf{0.028}} & \cellcolor{gray!60}\textbf{0.012} & \cellcolor{gray!30}{\textbf{0.025}} \\
\bottomrule
\end{tabular}%
}
\vspace{-2.8em}
\end{table}





